Crafter: Facial Feature Crafting against Inversion-based Identity Theft on Deep Models

With the increased capabilities at the edge (e.g., mobile device) and more stringent privacy requirement, it becomes a recent trend for deep learning-enabled applications to pre-process sensitive raw data at the edge and transmit the features to the backend cloud for further processing. A typical application is to run machine learning (ML) services on facial images collected from different individuals. To prevent identity theft, conventional methods commonly rely on an adversarial game-based approach to shed the identity information from the feature. However, such methods can not defend against adaptive attacks, in which an attacker takes a countermove against a known defence strategy. We propose Crafter, a feature crafting mechanism deployed at the edge, to protect the identity information from adaptive model inversion attacks while ensuring the ML tasks are properly carried out in the cloud. The key defence strategy is to mislead the attacker to a non-private prior from which the attacker gains little about the private identity. In this case, the crafted features act like poison training samples for attackers with adaptive model updates. Experimental results indicate that Crafter successfully defends both basic and possible adaptive attacks, which can not be achieved by state-of-the-art adversarial game-based methods.

==> tables/related.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
Three of the most prevailing attacks against user privacy is membership inference attack, attribute inference attack and model inversion attack. 
% Crafter targest the model inversion attack specifically, while existing baselines defend against different threat models.
 We compare Crafter with some most representative baselines in Table \ref{tab:comparison_realted} to further clarify the threat model in our scenario.

 Crafter and Adv Learning~\cite{xiao2020adversarial} specifically defend against model inversion attackers that are interested in the victim user's unknown identity. The attacker only has access to some public images that are non-overlapping with the user's identity, and intend to unveil the user's appearance via reconstruction. 
 
 Disco~\cite{singh2021disco} and TIPRDC~\cite{li2020tiprdc} defend both model inversion and attribute inference attacks that aim to attain the users private attributes (eg. age and gender). 
  Specifically, the attribute inference attacker trains an attribute classifer with an available training set. We change the sensitive attribute to `identity' in our evaluation against inversion attacks.

  Fawkes~\cite{shan2020fawkes} and LowKey~\cite{cherepanova2021lowkey} also defend against attribute inference attacks, but the private attribute of interest is identity.
  However, their identity attribute privacy is significantly different from our identity privacy against inversion attack. In LowKey and Fawkes, the attacker already has access to some of the victim's private images, on which it trains an attribute inference (facial recognition) attacker model  to infer the identity of the victim's other images. The defence is considered effective as long as the facial recognition attacker fails. In contrast, Crafter's attacker is interested in the appearance of an unknown victim, and the defence is robust only if the reconstructed image reveals no identity information percetually. Hence in Crafter, the facial recognition model merely serves as an oracle to evaluate the perceptual similarity between reconstructed and the raw images, but cannot be a real-world adversary model as private IDs of the training data are missing.
 

    \begin{table}[ht]
        \centering
        \small
        \caption{Comparison between Crafter and existing defences.}
        \label{tab:comparison_realted}
        \resizebox{\columnwidth}{!}{
        \begin{tabular}{cccc}
            \toprule
            Defense & Threat model & Privacy & Utility \\
            \midrule
            Crafter & \multirow{2}{*}{Model inversion} & \multirow{2}{*}{Identity} & Task oriented/agnostic \\ 
            AdvLearn~\cite{xiao2020adversarial} & & & Task oriented \\
            \cmidrule{1-4}
            Disco~\cite{singh2021disco} & Model inversion \& & \multirow{2}{*}{Attribute} & Task oriented \\
            TIPRDC~\cite{li2020tiprdc} & Attribute inference & & Task agnostic \\
            \cmidrule{1-4}
            Fawkes~\cite{shan2020fawkes} & Attribute inference & {Attribute} & \multirow{2}{*}{/}\\
            LowKey~\cite{cherepanova2021lowkey} & (Attribute=Identity) & (Identity)&  \\
            \bottomrule
        \end{tabular}
        }
    \end{table}
